Learning the Bitter Lesson: Empirical Evidence from 20 Years of CVPR Proceedings

This study examines the alignment of \emph{Conference on Computer Vision and Pattern Recognition} (CVPR) research with the principles of the "bitter lesson" proposed by Rich Sutton. We analyze two decades of CVPR abstracts and titles using large language models (LLMs) to assess the field's embracement of these principles. Our methodology leverages state-of-the-art natural language processing techniques to systematically evaluate the evolution of research approaches in computer vision. The results reveal significant trends in the adoption of general-purpose learning algorithms and the utilization of increased computational resources. We discuss the implications of these findings for the future direction of computer vision research and its potential impact on broader artificial intelligence development. This work contributes to the ongoing dialogue about the most effective strategies for advancing machine learning and computer vision, offering insights that may guide future research priorities and methodologies in the field.

==> tables/icc_results_tables.tex <==
\begin{table}[h]
\centering
\caption{ICC Results for learning_over_engineering_score}
\begin{tabular}{llrrrrrl}
\toprule
Type & Description & ICC & F & df1 & df2 & pval & CI95% \\
\midrule
ICC1 & Single raters absolute & 0.685000 & 7.536000 & 3997 & 7996 & 0.000000 & [0.67 0.7 ] \\
ICC2 & Single random raters & 0.686000 & 7.791000 & 3997 & 7994 & 0.000000 & [0.67 0.71] \\
ICC3 & Single fixed raters & 0.694000 & 7.791000 & 3997 & 7994 & 0.000000 & [0.68 0.71] \\
ICC1k & Average raters absolute & 0.867000 & 7.536000 & 3997 & 7996 & 0.000000 & [0.86 0.87] \\
ICC2k & Average random raters & 0.868000 & 7.791000 & 3997 & 7994 & 0.000000 & [0.86 0.88] \\
ICC3k & Average fixed raters & 0.872000 & 7.791000 & 3997 & 7994 & 0.000000 & [0.86 0.88] \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{ICC Results for search_over_heuristics_score}
\begin{tabular}{llrrrrrl}
\toprule
Type & Description & ICC & F & df1 & df2 & pval & CI95% \\
\midrule
ICC1 & Single raters absolute & 0.562000 & 4.849000 & 3997 & 7996 & 0.000000 & [0.55 0.58] \\
ICC2 & Single random raters & 0.569000 & 5.490000 & 3997 & 7994 & 0.000000 & [0.51 0.62] \\
ICC3 & Single fixed raters & 0.599000 & 5.490000 & 3997 & 7994 & 0.000000 & [0.58 0.62] \\
ICC1k & Average raters absolute & 0.794000 & 4.849000 & 3997 & 7996 & 0.000000 & [0.78 0.8 ] \\
ICC2k & Average random raters & 0.799000 & 5.490000 & 3997 & 7994 & 0.000000 & [0.75 0.83] \\
ICC3k & Average fixed raters & 0.818000 & 5.490000 & 3997 & 7994 & 0.000000 & [0.81 0.83] \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{ICC Results for scalability_with_computation_score}
\begin{tabular}{llrrrrrl}
\toprule
Type & Description & ICC & F & df1 & df2 & pval & CI95% \\
\midrule
ICC1 & Single raters absolute & 0.578000 & 5.112000 & 3997 & 7996 & 0.000000 & [0.56 0.59] \\
ICC2 & Single random raters & 0.586000 & 5.891000 & 3997 & 7994 & 0.000000 & [0.51 0.64] \\
ICC3 & Single fixed raters & 0.620000 & 5.891000 & 3997 & 7994 & 0.000000 & [0.6  0.63] \\
ICC1k & Average raters absolute & 0.804000 & 5.112000 & 3997 & 7996 & 0.000000 & [0.79 0.81] \\
ICC2k & Average random raters & 0.809000 & 5.891000 & 3997 & 7994 & 0.000000 & [0.76 0.84] \\
ICC3k & Average fixed raters & 0.830000 & 5.891000 & 3997 & 7994 & 0.000000 & [0.82 0.84] \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{ICC Results for generality_over_specificity_score}
\begin{tabular}{llrrrrrl}
\toprule
Type & Description & ICC & F & df1 & df2 & pval & CI95% \\
\midrule
ICC1 & Single raters absolute & 0.570000 & 4.983000 & 3997 & 7996 & 0.000000 & [0.55 0.59] \\
ICC2 & Single random raters & 0.578000 & 5.708000 & 3997 & 7994 & 0.000000 & [0.51 0.64] \\
ICC3 & Single fixed raters & 0.611000 & 5.708000 & 3997 & 7994 & 0.000000 & [0.6  0.63] \\
ICC1k & Average raters absolute & 0.799000 & 4.983000 & 3997 & 7996 & 0.000000 & [0.79 0.81] \\
ICC2k & Average random raters & 0.804000 & 5.708000 & 3997 & 7994 & 0.000000 & [0.76 0.84] \\
ICC3k & Average fixed raters & 0.825000 & 5.708000 & 3997 & 7994 & 0.000000 & [0.82 0.83] \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{ICC Results for favoring_fundamental_principles_score}
\begin{tabular}{llrrrrrl}
\toprule
Type & Description & ICC & F & df1 & df2 & pval & CI95% \\
\midrule
ICC1 & Single raters absolute & 0.010000 & 1.032000 & 3997 & 7996 & 0.126000 & [-0.01  0.03] \\
ICC2 & Single random raters & 0.181000 & 2.799000 & 3997 & 7994 & 0.000000 & [0.   0.35] \\
ICC3 & Single fixed raters & 0.375000 & 2.799000 & 3997 & 7994 & 0.000000 & [0.36 0.39] \\
ICC1k & Average raters absolute & 0.031000 & 1.032000 & 3997 & 7996 & 0.126000 & [-0.02  0.08] \\
ICC2k & Average random raters & 0.399000 & 2.799000 & 3997 & 7994 & 0.000000 & [0.01 0.62] \\
ICC3k & Average fixed raters & 0.643000 & 2.799000 & 3997 & 7994 & 0.000000 & [0.62 0.66] \\
\bottomrule
\end{tabular}
\end{table}



==> tables/krippendorff_alpha_results.tex <==
\begin{table}[h]
\centering
\caption{Krippendorff's Alpha Results}
\begin{tabular}{lcc}
\hline
Dimension & Alpha & Interpretation \\ \hline
Learning Over Engineering Score & 0.713 & Substantial \\
Search Over Heuristics Score & 0.513 & Moderate \\
Scalability With Computation Score & 0.578 & Moderate \\
Generality Over Specificity Score & 0.567 & Moderate \\
Favoring Fundamental Principles Score & -0.009 & Poor \\
\hline
\end{tabular}
\end{table}

==> tables/regression_results.tex <==
\begin{center}
\begin{tabular}{lclc}
\toprule
\textbf{Dep. Variable:}                           &  log\_citations  & \textbf{  R-squared:         } &     0.018   \\
\textbf{Model:}                                   &       OLS        & \textbf{  Adj. R-squared:    } &     0.017   \\
\textbf{Method:}                                  &  Least Squares   & \textbf{  F-statistic:       } &     14.90   \\
\textbf{Date:}                                    & Tue, 01 Oct 2024 & \textbf{  Prob (F-statistic):} &  1.62e-14   \\
\textbf{Time:}                                    &     21:05:55     & \textbf{  Log-Likelihood:    } &   -7398.7   \\
\textbf{No. Observations:}                        &        3967      & \textbf{  AIC:               } & 1.481e+04   \\
\textbf{Df Residuals:}                            &        3961      & \textbf{  BIC:               } & 1.485e+04   \\
\textbf{Df Model:}                                &           5      & \textbf{                     } &             \\
\textbf{Covariance Type:}                         &    nonrobust     & \textbf{                     } &             \\
\bottomrule
\end{tabular}
\begin{tabular}{lcccccc}
                                                  & \textbf{coef} & \textbf{std err} & \textbf{t} & \textbf{P$> |$t$|$} & \textbf{[0.025} & \textbf{0.975]}  \\
\midrule
\textbf{const}                                    &       4.0909  &        0.233     &    17.553  &         0.000        &        3.634    &        4.548     \\
\textbf{learning\_over\_engineering\_score}       &       0.0717  &        0.025     &     2.839  &         0.005        &        0.022    &        0.121     \\
\textbf{search\_over\_heuristics\_score}          &       0.0265  &        0.028     &     0.949  &         0.343        &       -0.028    &        0.081     \\
\textbf{scalability\_with\_computation\_score}    &       0.1140  &        0.036     &     3.185  &         0.001        &        0.044    &        0.184     \\
\textbf{generality\_over\_specificity\_score}     &      -0.0520  &        0.045     &    -1.155  &         0.248        &       -0.140    &        0.036     \\
\textbf{favoring\_fundamental\_principles\_score} &      -0.1894  &        0.042     &    -4.469  &         0.000        &       -0.272    &       -0.106     \\
\bottomrule
\end{tabular}
\begin{tabular}{lclc}
\textbf{Omnibus:}       & 30.247 & \textbf{  Durbin-Watson:     } &    1.430  \\
\textbf{Prob(Omnibus):} &  0.000 & \textbf{  Jarque-Bera (JB):  } &   38.751  \\
\textbf{Skew:}          & -0.119 & \textbf{  Prob(JB):          } & 3.85e-09  \\
\textbf{Kurtosis:}      &  3.422 & \textbf{  Cond. No.          } &     136.  \\
\bottomrule
\end{tabular}
%\caption{OLS Regression Results}
\end{center}

Notes: \newline
 [1] Standard Errors assume that the covariance matrix of the errors is correctly specified.
